Enhancing Noise Robustness of Parkinson's Disease Telemonitoring via Contrastive Feature Augmentation

Parkinson's disease (PD) is one of the most common neurodegenerative disorder. PD telemonitoring emerges as a novel assessment modality enabling self-administered at-home tests of Unified Parkinson's Disease Rating Scale (UPDRS) scores, enhancing accessibility for PD patients. However, three types of noise would occur during measurements: (1) patient-induced measurement inaccuracies, (2) environmental noise, and (3) data packet loss during transmission, resulting in higher prediction errors. To address these challenges, NoRo, a noise-robust UPDRS prediction framework is proposed. First, the original speech features are grouped into ordered bins, based on the continuous values of a selected feature, to construct contrastive pairs. Second, the contrastive pairs are employed to train a multilayer perceptron encoder for generating noise-robust features. Finally, these features are concatenated with the original features as the augmented features, which are then fed into the UPDRS prediction models. Notably, we further introduces a novel evaluation approach with customizable noise injection module, and extensive experiments show that NoRo can successfully enhance the noise robustness of UPDRS prediction across various downstream prediction models under different noisy environments.

==> data/relatedwork.tex <==
\section{Related Work}

\subsection{PD Telemonitoring} 

PD telemonitoring focuses on tracking the severity of the condition in individuals who have already been diagnosed with PD. Most works use the UPDRS as the primary evaluation metric. The PD telemonitoring task involves predicting UPDRS scores based on 16 speech measurement features extracted from PD patients.

Classical models, including the Least Absolute Shrinkage and Selection Operator (LASSO), Support Vector Machine (SVM) and Random Forest (RF) algorithm, have been utilized for prediction tasks \cite{tsanas2012accurate}. For SVM models, various Support Vector Regression (SVR), including the recently developed Householder transformation-based SVR, have been employed to predict UPDRS scores \cite{zhao2015householder}. To address the issue of data scarcity, a transfer learning approach has been proposed \cite{yoon2018novel}.

Recently, a hybrid ensemble learning method has been proposed, integrating SOM, Singular Value Decomposition (SVD), and ANFIS \cite{nilashi2019analytical}. First, SOM is utilized to group similar samples into distinct clusters. Second, SVD is applied for dimensionality reduction of input features, enabling data imputation and reducing the computational complexity of the subsequent ANFIS model. Third, ANFIS model is used to process the features with different membership functions and predict the UPDRS scores. Finally, an average ensemble strategy is employed to compute the final UPDRS scores. This approach achieves low prediction error and improved prediction performance while requiring less computation time. Similarly, other hybrid methods have been proposed, combining techniques such as SOM, GPR, and Laplacian Score \cite{nilashi2023parkinson}, or integrating EM, Principal Component Analysis (PCA), and neuro-fuzzy techniques \cite{nilashi2023early}.

\subsection{Feature Augmentation}

Feature augmentation is a technique that enhances the performance of machine learning models by expanding, modifying, or generating new features. It can be used in various scenarios. For probabilistic statistics, feature augmentation is used for sampling algorithms by introducing unobserved data or latent variables (e.g., EM and Latent Dirichlet Allocation). For image data, feature augmentation involves expanding the training dataset to prevent overfitting and enhance the model's robustness \cite{shorten2019survey}. For audio data, altering the speed of the audio signal serves as a technique for feature augmentation \cite{ko2015audio}. 

% For image data, feature augmentation involves expanding the training dataset to prevent overfitting and enhance the model's robustness. Simple transformations including flipping, color space augmentations and random cropping or erasing, other methods including noise injection, feature mixing, fake image generation and style transferring \cite{shorten2019survey}. For audio data, altering the speed of the audio signal serves as a technique for feature augmentation \cite{ko2015audio}.

Among the various proposed feature augmentation approaches, Contrastive Learning (CL) has emerged as a powerful approach, effective for leveraging unlabeled data. CL has been employed to perform data augmentation for images \cite{xiao2020should}. Graph-structured data also benefits from specialized CL methods, including spectral graph contrastive learning \cite{zhang2023spectral} and graph meta-learning \cite{zhu2021graph}. A supervised Label Informed Contrastive Pretraining (LICAP) method employs CL to hierarchically distinguish high-importance nodes in knowledge graphs \cite{zhang2024label}.

In PD diagnosis task, a CL-based self-supervised multimodal (i.e., hand-drawing, speech, and gait) feature augmentation method achieves state-of-the-art performance \cite{wang2023analysis}. Note that, the above PD diagnosis task is binary classification. However, our CL-based feature augmentation method focuses on PD telemonitoring, which is a regression task for UPDRS scores with only speech features. By learning robust representations through the CL feature augmentation method, our prediction framework NoRo aligns feature distributions between clean and noisy conditions, mitigating sensitivity to measurement noise, thereby enhancing noise robustness and reliability in PD telemonitoring scenarios.

% While LICAP is originally designed for graph-structured data, its CL framework exhibits transferable potential for improving noise robustness in UPDRS prediction tasks. Moving beyond LICAP’s supervised label dependency, a ‌self-supervised feature augmentation method‌ based on CL is proposed to enhance noise robustness for prediction models. 

% \subsection{Applications of CL}

% CL is a self-supervised machine learning method designed to enhance model performance by leveraging large amounts of unlabeled data. Its object is to bring similar samples closer together in the feature space while pushing dissimilar samples further apart.

% CL is widely used to enhance feature representations in classification tasks. For image classification, robust CL methods have been proposed, achieving performance comparable to that of supervised learning\cite{wang2022contrastive}. Additionally, supervised contrastive loss has been introduced, enabling simultaneous learning of feature representations and classification \cite{wang2021contrastive}. In few-shot learning (FSL), CL has been incorporated into both the pretraining and meta-training stages, resulting in significant performance improvements for few-shot classification models\cite{yang2022few}.

% CL is also applied in PD diagnosis. For example, a CL framework leveraging large amounts of unlabeled data for data enhancement has demonstrated superior performance in multimodal scenarios\cite{wang2023analysis}. Additionally, CL has been utilized in graph convolutional networks for PD diagnosis, using a toe-tapping dataset\cite{guo2022contrastive}, and for fine-grained feature extraction from hand movement data, leading to the development of a new PD assessment metric\cite{guo2022tree}.

% CL can also be applied to solve regression problems, although it has mostly been used in classification tasks. A label informed contrastive pretraining (LICAP) method has been proposed for node importance estimation in knowledge graphs, incorporating CL to distinguish top nodes with higher importance from non-top nodes\cite{zhang2024label}. To enhance performance, samples within the top nodes are further organized into additional bins based on labels, and CL is used to differentiate nodes within each bin. Similar to LICAP, the proposed feature enhancement method groups samples into different bins based on feature dimensions, which is an unsupervised learning approach to improve the robustness against noise in predictions.

==> data1/experiment.tex <==
\section{Experimental Settings}

\subsection{Dataset}

The PD telemonitoring dataset of UCI is used in this work\cite{misc_parkinsons_telemonitoring_189}, also used in other related works\cite{nilashi2019analytical, nilashi2023parkinson, zhao2015householder, nilashi2023early}.

This dataset contains a total of 5875 speech test samples collected from 42 PD patients through multiple measurements. Each sample includes 2 labels, Motor UPDRS and Total UPDRS, along with 16 speech features, \{Jitter(\%)\}, \{Jitter(Abs)\}, \{Jitter:RAP\}, \{Jitter:PPQ5\}, \{Jitter:DDP\}, \{Shimmer\}, \{Shimmer(dB)\}, \{Shimmer:APQ3\}, \{Shimmer:APQ5\}, \{Shimmer:APQ11\}, \{Shimmer:DDA\}, \{NHR\}, \{HNR\}, \{RPDE\}, \{DFA\}, \{PPE\}.

The data were divided into a training set and a testing set. A 10-fold leave-one-out cross-validation approach was employed in this study. The number of samples in each set is presented in Table\ref{tab:Dataset_Split}, consistent with the dataset used in \cite{zhao2015householder}, with the addition of a validation step. The model exhibiting the lowest loss during the validation step is preserved.

\begin{table}[htbp]
    \centering
    \caption{Dataset Split}
    \renewcommand\tabcolsep{3.8pt}
    \renewcommand{\arraystretch}{1.5}
    \scalebox{0.8}
    {
        \begin{tabular}{cccc}
            \toprule
            Label & Training & Valid & Test \\
            \midrule
            Motor UPDRS   & 2700 &300 & 2875 \\
            Total UPDRS   &  2700 &300 & 2875 \\
            \bottomrule
        \end{tabular}
        \label{tab:Dataset_Split}
    }
\end{table}

Due to significant differences in the magnitudes of the speech features, such as the feature \{Jitter(\%)\} having an order of magnitude of $10^{-3}$, the feature \{Jitter(Abs)\} ranging from $10^{-5}$ to $10^{-6}$, and the feature \{HNR\} reaching an order of magnitude of $10^1$, a z-score normalization step is necessary before conducting experiments, as illustrated in Equation\ref{eq:zscore},

\begin{equation}
    \centering
    x_{ij} \leftarrow \frac{x_{ij}-\overline{x_j}}{\sigma_{x_j}},
    y_{i} \leftarrow \frac{y_{i}-\overline{y}}{\sigma_{y}}
    \label{eq:zscore}
\end{equation}

where $x_{ij}$ is the $j$th feature of the $i$th sample, $\overline{x_j}$ and $\sigma_{x_j}$ are the mean and the standard deviation of the $j$th feature across all samples, respectively. The normalization of label $y$ is similar to that of $x$.

The normalization step is also consistent with \cite{zhao2015householder}. The same normalization procedure is applied to the testing dataset using the same mean and standard deviation values obtained from the training dataset.

\subsection{Noise Setting}

To simulate a real-world noisy environment, random Gaussian noise $N$ is added to the voice feature $X$ to create the noisy feature $Z=X+N$\cite{mivule2013utilizing}.

To generate random Gaussian noise $N$, a mean value of ${\mu}=0$ is selected and the variance is determined based on the given signal-to-noise ratio (SNR).

SNR is expressed in decibels (dB). The higher the SNR, the less the signal is affected by noise, indicating better signal quality. The realtionship between the signal and noise power is given by 

\begin{equation}
    {SNR} = 10 ~ log_{10} ~ ({\frac{P_X}{P_N}})
\end{equation}

, where $\mathbf{P_X}$ is the power of the original voice feature, $\mathbf{P_N}$ is the power of the noise.

$\mathbf{P_X}$ is estimated by the following equation

\begin{equation}
    {P_{X_j}} = \frac{1}{n} \sum_{i=1}^{n} {X_{ij}}^{2}
\end{equation}

, where ${P_{X_j}}$ is the power of the $j$th feature, and $n$ is the total number of the samples. This equation indicates that the power of the $j$th feature is represented as the mean of the square of the $j$th original feature across all samples.

Because the power $P_N$ of Gaussian noise with ${\mu}=0$ equals its variance ${\sigma}^2$, the variance of the Gaussian noise $\boldsymbol{\sigma^2}$, is given by 

\begin{equation}
    {\sigma_j}^2 = {P_{X_j}} \cdot 10^{-\frac{SNR}{10}}
\end{equation}

\subsection{Evaluation}

\subsubsection{Baseline}



\subsubsection{Metrics}

In this study, prediction errors are evaluated using root mean square error (RMSE), mean absolute error (MAE)\cite{nilashi2019analytical,zhao2015householder}, and median absolute error (MedianAE)\cite{zhang2024label}, as defined by Equation \ref{eq:RMSE}, \ref{eq:MAE}, and \ref{eq:MedianAE}, respectively.

\begin{equation}
    RMSE = \sqrt{\frac{1}{n}\sum_{i=1}^{n}{(y_i-\widehat{y_i})}^2}
    \label{eq:RMSE}
\end{equation}

\begin{equation}
    MAE = \frac{1}{n}\sum_{i=1}^n \left|y_i-\widehat{y_i}\right|
    \label{eq:MAE}
\end{equation}

\begin{equation}
    MedianAE = median\{\left|y_i-\widehat{y_i}\right|,i=1,2,\ldots,n\}
    \label{eq:MedianAE}
\end{equation}

The smaller these metrics, the better the prediction of UPDRS.

\subsection{Implementation Details}

\subsubsection{Feature Selection}

As mentioned in Section \ref{section:overview}, a random forest feature selection algorithm is used to determine the specific binning feature $X_i$ by assessing the importance of each feature dimension.

Ramdom forest regression is an ensemble learning method that evaluates the importance of each feature by calculating its contribution across all decision trees.

Random forest regression was utilized to select features with higher variable importance score, which guided the initialization of the search process for the second step in indentifying computer security threats and ultimately increased classification accuacy\cite{hasan2016feature}.

In this study, random forest is also employed to evaluate the importance score of each feature dimension for both Motor UPDRS and Total UPDRS. After 10 replications, the average importance scores for each feature dimension are illustrated in Figure \ref{fig:random forest}.

\begin{figure}
    \centering

    \subfigure[Motor UPDRS]
    	{\includegraphics[width=0.5\textwidth]{Figs/Experiment/Feature Selection 1.png}}

    \subfigure[Total UPDRS]
    	{\includegraphics[width=0.5\textwidth]{Figs/Experiment/Feature Selection 2.png}}

    \caption{Importance Scores by Random Forest}
    \label{fig:random forest}
\end{figure}

Therefore, the most important feature dimensions, namely \{DFA\}, \{HNR\}, and \{Jitter(Abs)\}, are selected.

\subsubsection{Hyperparameter}



\subsubsection{Experimental environment}

The experiments can be conducted on both Windows and Linux operating systems. The proposed code is developed based on Pytorch and the machine learning library scikit-learn. The environment configuration is shown in Table \ref{tab:Environment Configuration}.

\begin{table}[]
    \centering
    \caption{Environment Configuration}
    \renewcommand\tabcolsep{3.8pt}
    \renewcommand{\arraystretch}{1.5}
    \scalebox{0.8}
    {
        \begin{tabular}{c|cc}
            \toprule
               Name & Version & Build\\
               \midrule
                python & 3.9.15 & h4de0772\_0\_cpython\\
                torch & 1.13.0+cu117 & pypi\_0 \\
                torchvision & 0.14.0+cu117 & pypi\_0 \\
                cuda & 12.1 & 0\\
                scikit-learn & 1.1.3 & pypi\_0 \\
                \bottomrule
            \end{tabular}
            \label{tab:Environment Configuration}
    }
\end{table}

==> data1/introduction.tex <==
\section{Introduction}

Parkinson's disease (PD) is recognized as a complex neurodegenerative disorder\cite{kalia2015parkinson}. Apart from the its pathological characteristics, PD also presents with a large number of clinical characteristics where the motor features, including rest tremor, bradykinesia, rigidity, and loss of postural reflexes are considered the cardinal signs of PD\cite{jankovic2008parkinson}. Except for infectious causes, aging, genetic, and environmental factors, such as pesticide exposure, dairy product consumption, a history of melanoma, and traumatic brain injury, can all contribute to the development of PD\cite{ascherio2016epidemiology,bloem2021parkinson}.

PD is the most common age-related neurodegenerative disorder after Alzheimer's disease. Aging is the most significant risk factor for PD. Therefore, with the aging population, the prevalence of PD would rise gradually, resulting in more severe health and economic issues for society\cite{reeve2014ageing}. More specifically, the prevalence of PD is more than 1\% among individuals over the age of 60 by the year of 2004 while over 1 million people in North America were diagnosed with PD by the year of 1998\cite{samii2004parkinson, ae1998parkinson}. In China, there were nearly 3 million individuals with PD, accounting for half of the global patient population, and is increasing of about 0.1 million cases annually.

Measuring the progression of PD has attracted the attention of scholars worldwide. In addition to various methods based on the pathological characteristics-such as assessing the content of  $\alpha$-synuclein-containing Lewy bodies or the infiltration of the Lewy bodies in the brain-clinical scales, such as Unified Parkinson’s Disease Rating Scale (UPDRS) are also employed to capture clinical features of PD like bradykinesia, rigidity, and tremor\cite{halliday2010progression, poewe2009clinical}.

However, tracking PD progression typically requires patients' presence in the hospital. Due to motor symptoms such as movement disorders and gait difficulties, frequent hospital visits can be inconvenient for PD patients. Currently, a non-invasive telemonitoring method for PD allows them to conduct their own PD progression assessments at home, freeing them from the burden of frequent hospital visits, and is more cost-effective. If widely adopted, this approach could also alleviate the workload on hospitals, and healthcare providers\cite{tsanas2009accurate}. 

This approach utilizes Intel Corporation's At-Home Testing Device (AHTD) to record the voice data of PD patients, aiming to measure PD-related motor impairment symptoms\cite{goetz2009testing}. Through speech signal processing algorithms, 16 features are extracted from the patients' speech characteristics, which can then be mapped to the UPDRS scores\cite{tsanas2009accurate}. The UPDRS is a reliable and valid clinical rating scale for PD, widely utilized to assess the progression of it and nearly comprehensive in its coverage of motor symptoms\cite{movement2003unified}. The motor and total UPDRS scores are the most closely related to speech characteristics of PD patients\cite{nilashi2018hybrid}.

There are many studies utilize these speech features to predict UPDRS scores. Most studies use hybrid architectures for the prediction task. Hybrid systems composed of clustering methods such as self-organizing map (SOM) and expectation maximization (EM), along with regression methods such as Gaussian process regression (GPR) and adaptive network-based fuzzy inference system (ANFIS), have been proposed\cite{nilashi2019analytical,nilashi2023parkinson, zogaan2024combined, vats2023predicting}.

However, since PD patients need to use the AHTD to conduct speech tests at home without professional supervision, noise can be introduced into the test results. For example, the AHTD requires PD patients to keep their mouths approximately 5 centimeters away from the microphone and to produce vowels at a consistent frequency\cite{goetz2009testing}. Additionally, environmental noise can interfere with the speech test results\cite{nicastri2004multidimensional}. Besides, in terms of data processing, the collected data needs to be encrypted and transmitted to a server, where it is processed using speech signal processing algorithms. During data transmission or decryption, packet loss or decryption failures may occur\cite{goetz2009testing}.

Although previous research has achieved some success in PD telemonitoring, including reducing prediction errors\cite{nilashi2023parkinson} and improving computation speed\cite{nilashi2019analytical}, it generally overlooks these noise issues. To address these issues, a feature enhancement methods is proposed in this work to improve the robustness of prediction algorithms to noise, mitigating the decline in prediction performance caused by noise.

The main contributions of this work are as follows.
\setlist{nolistsep}
\begin{itemize}[noitemsep]
	\item A feature enhancement method based on contrastive learning (CL) is proposed to improve the robustness of various prediction algorithms to noise. This method can aid in expanding the use of PD telemonitoring, thereby benefiting a large number of PD patients. Furthermore, this work is pioneering in the field of PD telemonitoring as it addresses the practical issue of the robustness of prediction methods to noise.
	
	\item The proposed method is flexible and can be easily integrated into other feature vector-based PD assessment systems. It also provides a method for improving robustness that can be applied to other diagnostic scenarios where noise is a significant issue.
	
	\item The proposed method is validated across various prediction algorithms, including classical methods(multiple linear regression (MLR), support vector regression (SVR)), neural networks (NN), ensemble methods (AdaBoost), as well as GPR and ANFIS.
	
	\item The proposed method is evaluated using a real-world PD telemonitoring dataset from the Machine Learning Repository at the University of California, Irvine (UCI)\cite{misc_parkinsons_telemonitoring_189}, which is widely used for UPDRS prediction.
\end{itemize}

==> data1/method.tex <==
\section{Methodology}\label{method}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.995\linewidth]{Figs/Method/Overview.png}
	\caption{An overview of the proposed model.}
	\label{fig:overview}
\end{figure*}

\subsection{Problem Formulation}

Given the speech feature $X$ and noise $N$, the noisy feature is represented as $Z=X+N$.

\begin{mydef}
	(Feature Enhancement): Feature enhancement refers to using a machine learning model $F$ to project $X$ or $Z$ into an enhanced feature space as $X'=F(X)$ and $Z'=F(Z)$
\end{mydef}

\begin{mydef}
	(Robustness): The robustness of a regression model refers to its ability to withstand noise, mitigating the decline in prediction performance caused by $N$.
\end{mydef}

The goal of the feature enhancement is to reduce the error in predicting $Z'$ using the model, making it smaller than the error in predicting $Z$.

\subsection{Overview}
\label{section:overview}

 Figure \ref{fig:overview} illustrates the overview of the proposed model, which consists of two general parts:

First is the feature enhancement part. CL is employed in this part to train a multilayer perceptron (MLP). This MLP is used to map $X$ and $Z$ into the enhanced feature space, forming the enhanced feature vectors $X'$ and $Z'$. For the generation of positive and negative pairs, each feature vector was assigned to the corresponding bin based on a specific dimension $X_i$, which is chosen by a random forest feature selection algorithm. 

Second is the prediction part. Various regression models are used to predict UPDRS based on the enhanced features $Z'$ instead of only original features $Z$. To achieve better performance, $Z'$ can be concatenated with $Z$ for prediction.

\subsection{Model Design}

An initial binning of the features is proposed in this work to enhance the model's robustness against noise, followed by feature enhancement based on the binning results. The advantage of this approach is that even if the original feature vectors are affected by the noise, it is less likely to cause significant deviations in the enhanced feature space or result in shifts into other bins. This method helps preserve the robustness of the feature vectors within their respective bins and, consequently, improves the robustness of the prediction models.

\subsubsection{Binning Method}
\label{section:Binning}

To enhance the robustness of the model, equal-width binning is applied to $X_i$. The range of $X_i$ is divided into intervals of equal width. 

However, as shown in Figure \ref{fig:overview}, bin centers are essential for generating positive and negative pairs. But when the number of bins is large, some bins may not contain any feature vectors, making it impossible to calculate the bin center. 

For these bins that do not contain any feature vectors, the bin center is represented by the bin center of the nearest non-empty bin. If there are two nearest non-empty bins, the bin center is represented by the average of their bin centers.

\subsubsection{Loss Function}

To perform feature enhancement based on binning results, contrastive learning is employed in this work, bringing feature vectors within the same bin closer together while pushing feature vectors from different bins farther apart in the enhanced feature space.

The loss function used for the MLP in feature enhancement is the contrastive loss, as shown in Equation \ref{eq:CLLoss}:

\begin{equation}
	L = -\sum_{i=1}^{N_{bin}}\sum_{j\in bin_i} log{\frac{\exp{(h_j c_i)}}{\sum_{k=1}^{N_{bin}} \exp{(\alpha_{ik}h_j c_k)}}}
	\label{eq:CLLoss}
\end{equation}
, where $h_j$ represents the projection of the $j$-th feature vector in the enhanced feature space, $N_{bin}$ denotes the total number of bins, and $c_i$ represents the bin center of the $i$-th bin, which is defined as the average of all enhanced feature vectors within this bin.

Considering that bins are closer to each other have a stronger correlation, a distance coefficient is introduced to represent this relationship, which increases as the distance between bins decreases. $\alpha_{ik}$ represents the distance coefficient between the $i$-th and the $k$-th bin. 

For each bin, the distance coefficient is the same for all bins that are equidistant from it. Therefore, for the $m$-th bin, the distribution of the distance coefficient needs to be symmetric around $m$, as illustrated in Figure \ref{fig:alpha-bin}.

\begin{figure}
	\centering
	\includegraphics[width=0.995\linewidth]{Figs/Method/Figure3_2.png}
	\caption{Distance Coefficients for the $m$-th Bin}
	\label{fig:alpha-bin}
\end{figure}

For the design of this distribution, a normalized modified binomial distribution is applied in this work\cite{zhang2024label}. The distance coefficient between the $m$-th and the $n$-th bin is shown in Equation \ref{eq:cal alpha}:

\begin{equation}
	\centering
	{\alpha}_{mn}={\alpha}_{nm}=\frac{\binom{N}{n-m+N/2}}{\binom{N}{N/2}}
	\label{eq:cal alpha}
\end{equation}
, where $N$ is an even number to ensure the distribution function has a single maximum value, which occurs when $m=n$, expressed as $N=2~max(m, N_{bin}-m)$. Further normalization is applied to ensure the distribution reaches its maximum value of 1 when $m=n$. Due to the properties of binomial coefficients, this distribution is symmetric with respect to $m$.

\subsection{Algorithm and Implementation}

The training algorithm is shown in Algorithm \ref{alg:training}:

%\renewcommand{\algorithmicrequire}{\textbf{Input：}\unskip}
%\renewcommand{\algorithmicensure}{\textbf{Output：}\unskip}

\begin{algorithm}
	\caption{Feature Enhancement Model Training Algorithm}
	\label{alg:training}
	\small
	\begin{algorithmic}[1]
		\Require Feature Vector Matrix $X$; Bin Number $N_{bin}$
		\Ensure Parameters of the Feature Enhancement MLP $W$
		
		\State Select the binning vector $X_i$
		\State Perform binning based on $X_i$
		\State Calculate distance coefficients $\{{\alpha}_{11},\ldots,{\alpha}_{N_{bin}N_{bin}}\}$
		\State Initialize $W$
		
 		\For{$epoch$ = 1 to $epochs$}
			\For{$bin_i$ in $\{bin_1,bin_2,\ldots, bin_{N_{bin}}\}$}
				\State Calculate $c_i$
			\EndFor
			\State Initialize loss $L=0$
			\For{Feature vector $i$ in $X$}
				\State $h_i \leftarrow \sigma(W X_i)$
				\State $L_i \leftarrow -log{\frac{\exp{(h_i c_i)}}{\sum_{k=1}^{N_{bin}} \exp{(\alpha_{ik}h_i c_k)}}}$
				\State $L \leftarrow L+L_i$
			\EndFor
			\State Update $W$ by minimizing $L$ using gradient descent
		\EndFor
		\Return $W$
	\end{algorithmic}
\end{algorithm}

%\subsection{Algorithm and Implementation}
%Finally, we summarize the overall algorithm and analyze its complexity.
%\begin{algorithm}[htbp]
%\caption{KGC-Explainer} \label{alg1}
%\textbf{Input}: attributed biased transition matrix $T$, walks per node $r$, walk length $l$, window size $w$, embedding dimensionality $d$
%\\ \textbf{Output}: node embedding matrix $Z \in \mathbb{R}^{n \times d}$
%\begin{algorithmic}[1] %[1] enables line numbers
%\State Initialize a list $walks=[~]$
%\For{$iter\in r$} \Comment{parallel}
%    \For{$v_i\in\mathcal{V}$ } \Comment{parallel}
%        \State Initialize a list $walk=[v_i]$
%        \For{$walk\_iter\in l$ }
%            \State $curr\_node=walk[-1]$
%            \State $prob\_dist = T_{curr\_node}$
%            \State $next\_node = AliasSampling(prob\_dist)$
%            \State Append $next\_node$ to $walk$
%        \EndFor
%        \State Append $walk$ to $walks$
%    \EndFor
%\EndFor
%\State obtain $Z \in \mathbb{R}^{n \times d}$ by training $word2vec(walks,w,d)$
%\State \textbf{return} node embedding matrix $Z \in \mathbb{R}^{n \times d}$
%\end{algorithmic}
%\end{algorithm}

